Femto-Containers: DevOps on Microcontrollers with Lightweight Virtualization & Isolation for IoT Software Modules

Development, deployment and maintenance of networked software has been revolutionized by DevOps, which have become essential to boost system software quality and to enable agile evolution. Meanwhile the Internet of Things (IoT) connects more and more devices which are not covered by DevOps tools: low-power, microcontroller-based devices. In this paper, we contribute to bridge this gap by designing Femto-Containers, a new architecture which enables containerization, virtualization and secure deployment of software modules embedded on microcontrollers over low-power networks. As proof-of-concept, we implemented and evaluated Femto-Containers on popular microcontroller architectures (Arm Cortex-M, ESP32 and RISC-V), using eBPF virtualization, and RIOT, a common operating system in this space. We show that Femto-Containers can virtualize and isolate multiple software modules, executed concurrently, with very small memory footprint overhead (below 10%) and very small startup time (tens of microseconds) compared to native code execution. We show that Femto-Containers can satisfy the constraints of both low-level debug logic inserted in a hot code path, and high-level business logic coded in a variety of common programming languages. Compared to prior work, Femto-Containers thus offer an attractive trade-off in terms of memory footprint, energy consumption, agility and security.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> Text/4a-bpf-additional-background.tex <==
\section{Additional Background on eBPF Virtualization}
The virtual machine operates on 11 registers of 64 bits.
The last register (\texttt{r10}) is a read-only pointer to the beginning of a \SI{512}{\byte} stack.
Interaction with the stack happens via load and store instructions as shown in \autoref{fig:isa}.
% moving values from the registers to the stack and vise versa.
Instructions are divided into an \SI{8}{\bit} opcode, two \SI{4}{\bit} registers: source and destination, an \SI{16}{\bit} offset field and an \SI{32}{\bit} immediate value.
Unused fields in an instruction are set to zero.
Position-independent code is achieved by using the reference in \texttt{r10} and the offset field in the instructions.

\begin{figure}[t]
  \centering
    \includegraphics[width=\columnwidth]{Figures/isa.pdf}
  \caption{eBPF instructions, registers and stack.}
  \label{fig:isa}
\end{figure}

%Most instruction do not use all fields, the fields not used for an instruction must be zero.

==> Text/5-experimental-setup.tex <==
\section{Experimental setup}

We carry out our measurements on popular, commercial off-the-shelf IoT hardware: a Nordic nRF52840 Development Kit, which provides a typical microcontroller (Arm Cortex-M4) with 256 KB RAM, 1 MB Flash, and a 2.4 GHz radio transceiver compatible both with IEEE 802.15.4, and Bluetooth Low-Energy.
This hardware is also available for reproduceability on open access testbeds such as IoT-Lab~\cite{iot-lab2015-ieee-iot-wf}.

On this platform, we perform two types of benchmarks.
First, we perform embedded computing hosted in the VM, to get an idea of basic VM performance.
Then, we perform further benchmarks involving IoT networking capabilities used from within the \ac{VM}.

\subsection{Computing Benchmark Setup}

First, we benchmark a setup consisting of a Fletcher32 checksum algorithm~\cite{fletcher}.
The Fletcher32 checksum algorithm requires a mix of mathematical operations memory reads and branches, containing a loop over input data.
Benchmark results consist of the impact of the \ac{VM} on the operating system in the additional memory required to include it.
For the \acp{VM} themselves, the execution speed and the size of compiled applications loaded into the \ac{VM} is measured.

\if{0}
binary statistics: %See `llvm-objdump -d fletcher32_bpf.o`
\begin{itemize}
\item 61 instructions
\item 3 double word loads (128 bit wide instructions (LLDW))
\item 4 branch instructions and single return
\item 4 loads of which 2 in the main loop.
\item the rest is arithmetic
\end{itemize}
\fi


\subsection{Networked Benchmark Setup}

Next, we construct a setup involving a simple IoT networked application as case study.
The \ac{VM} hosts high-level logic, and this loaded application is updateable over the network.
The functionality mimics that studied in prior work~\cite{riot-js-container} using small JavaScript run-time containers hosting application code on top of RIOT\@.
The hosted logic has access to both the CoAP stack and the high-level sensor interface (SAUL) provided by  RIOT~\cite{baccelli2018riot}.
The VM execution is triggered by a CoAP request and the operating system expects a formatted CoAP response payload or an error code from the application loaded in the \ac{VM}.
The goal is to load an application into the \ac{VM} that, when triggered by a CoAP request, reads a sensor value and constructs a full CoAP payload as response to the requester.


==> Text/background.tex <==
\section{Background}

\subsection{WebAssembly}
WebAssembly (Wasm~\cite{haas2017wasm}) is a virtual instruction set architecture, standardized by the World Wide Web Consortium (W3C), primarily aimed at portable web applications.
The instruction set allows for binaries small in size, to minimize transfer time to the client.
The sandbox provided by implementations offers strong guarantees on memory access.
Both of these properties aim to ensure security while requiring only limited memory footprint on the platform target.

The WebAssembly \ac{VM} uses both a stack and a flat heap for memory storage.
The stack is required by the architecture, and can be configured to any size.
An interface for allocating heap memory is provided by the standard.
Specification mandates memory allocations in chunks of \SI{64}{\kibi\byte} (pages).
%which is not always possible on smaller IoT platforms.

{\bf Toolchain \& SDK}. %A software development kit is available to write applications for WebAssembly.
The full workflow for development and execution of Wasm applications is depicted in \autoref{fig:wasm3_workflow}.
Wasm uses the LLVM compiler: applications in any language supported by LLVM are possible, such as C/C++, D, Rust, and TinyGo among others.
%Note that for C and C++, the WebAssembly binaries are created using the emcc toolchain, which combines the EmSDK with LLVM\@.
A standardized interface is specified for host access in a POSIX-like way is provided by the WASI standard~\cite{WASI}.
%It offers standardized access to operating system facilities such as files, network sockets, clocks and random number.

{\bf Interpreter.} Once the Wasm binary is created, it can be transferred to the IoT device,
on which it is interpreted and executed, as shown in \autoref{fig:wasm3_workflow}.
Several interpreters exist,
in this paper we use the WASM3~\cite{wasm3} interpreter,
which uses a two-stage approach: the loaded application is first transpiled to an optimized executable, which then can be executed in the interpreter.

\begin{figure}
  \centering
  \includegraphics[width=0.8\linewidth]{wasm3_workflow}
  \caption{Wasm code development and execution workflow with the WASM3 \ac{VM}.}
  \label{fig:wasm3_workflow}
  \vspace{-1.5em}
\end{figure}

\subsection{Extended Berkeley Packet Filters}

Berkeley Packet Filter (BPF~\cite{fleming2017eBPF}) is a small in-kernel \ac{VM} available on most Unix-like operating systems.
Its original purpose was network packet filtering, for example: only pass to userspace packets matching a set of requirements.
Within the Linux kernel the \ac{VM} is extended (to eBPF) to allow for multiple non-network related purposes.
eBPF provides a small and efficient facility for running custom code inside the kernel, hooking into various subsystems.

The state-of-the-art eBPF architecture is 64-bit register based \ac{VM} with a fixed stack.
%10 general purpose registers are available together with a read-only stack pointer.
The stack itself is specified as fixed at \SI{512}{\byte}.
A heap is not contained in the specification. As an alternative, the Linux kernel provides an interface to key-value maps for persistent storage between invocations.
%These maps can also be interfaced with from user space applications.
The limited stack size and absence of a heap put only minimal requirements on the RAM a platform has to provide for the \ac{VM}.

\begin{figure}
\centering
\includegraphics[width=0.8\linewidth]{rbpf_workflow}
\caption{rBPF code development and execution workflow.}
\label{fig:rbpf_workflow}
\vspace{-1.5em}
\end{figure}

The \ac{VM} itself is inherently suitable for isolating the operating system from the virtualized application:
all memory access, including to the stack, happen via load and store instructions.
Moreover, branch and jump instructions are also limited, the application has no access to the program counter and a jump is always direct and relative to current program counter.
The \ac{VM} does not provide facilities to directly write the program counter.
Both of these potential attack surfaces can be implemented with the necessary checks in place to limit access and execution.

Interfacing with the operating system facilities can be done by providing the necessary bindings on the device.
%These can then be accessed during execution from the \ac{VM}. 
%Function calls, both within the applications and to operating system bindings happen through a call instruction and register zero through 4 are used as implicit arguments to the function.
%The return value is stored in register zero before returning.

% Wasm vs BPF
{\bf Comparing eBPF to WebAssembly.}
As with WebAssembly, eBPF makes use of the LLVM toolchain for compilation (see \autoref{fig:rbpf_workflow}) thus any language supported by LLVM can be used and compiled to bytecode.
However, there are differences in terms of architecture, and in terms of memory model.
The architecture of WebAssembly reduces the size of instructions significantly.
On the other hand, eBPF instructions are always \SI{64}{\bit} in size, filled with zero bits where a field is not used.
The stack-based with heap memory approach from WebAssembly put significant requirements on the available RAM\@.
On the other hand, with eBPF, the few registers combined with the limited stack put only minimal pressure on the available RAM\@.
% closing remark? script size vs memory requirement?

